Vulnerability Detection: From Formal Verification to Large Language Models and Hybrid Approaches: A Comprehensive Overview

Software testing and verification are critical for ensuring the reliability and security of modern software systems. Traditionally, formal verification techniques, such as model checking and theorem proving, have provided rigorous frameworks for detecting bugs and vulnerabilities. However, these methods often face scalability challenges when applied to complex, real-world programs. Recently, the advent of Large Language Models (LLMs) has introduced a new paradigm for software analysis, leveraging their ability to understand insecure coding practices. Although LLMs demonstrate promising capabilities in tasks such as bug prediction and invariant generation, they lack the formal guarantees of classical methods. This paper presents a comprehensive study of state-of-the-art software testing and verification, focusing on three key approaches: classical formal methods, LLM-based analysis, and emerging hybrid techniques, which combine their strengths. We explore each approach's strengths, limitations, and practical applications, highlighting the potential of hybrid systems to address the weaknesses of standalone methods. We analyze whether integrating formal rigor with LLM-driven insights can enhance the effectiveness and scalability of software verification, exploring their viability as a pathway toward more robust and adaptive testing frameworks.

==> main <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{staticanalysis2022}
\citation{IAST}
\citation{fuzzing}
\citation{pentest}
\citation{Formalverification}
\providecommand \oddpage@label [2]{}
\@writefile{toc}{\contentsline {title}{Vulnerability Detection with LLMs and FV tools}{1}{chapter.1}\protected@file@percent }
\@writefile{toc}{\authcount {7}}
\@writefile{toc}{\contentsline {author}{N.Tihanyi et al.}{1}{chapter.1}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.1.1}\protected@file@percent }
\citation{RASP}
\citation{LLMfuzz}
\citation{invariants}
\citation{tihanyi_how_2024}
\citation{wang2024your}
\citation{roychoudhury2025ai}
\citation{lyu2024automatic}
\citation{BMCfirst}
\citation{10.1145/3650212.3685304}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces High-level categories of Software Testing}}{2}{figure.caption.2}\protected@file@percent }
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{fig:Maincategories}{{1}{2}{High-level categories of Software Testing}{figure.caption.2}{}}
\citation{10825051}
\@writefile{toc}{\contentsline {section}{\numberline {2}Motivation}{3}{section.1.2}\protected@file@percent }
\citation{ESBMC}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Motivating examples posing challenges for LLMs an FV tools }}{4}{figure.caption.3}\protected@file@percent }
\newlabel{fig:motivation}{{2}{4}{Motivating examples posing challenges for LLMs an FV tools}{figure.caption.3}{}}
\citation{sheng2025large}
\citation{MECHRI2025104151}
\citation{sheng2025large}
\citation{jiang2024investigating}
\citation{hanif2022vulberta}
\citation{ferrag2023securefalcon}
\citation{du2024generalization}
\citation{zhou2024large}
\@writefile{toc}{\contentsline {section}{\numberline {3}LLMs in Vulnerability Detection}{5}{section.1.3}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}Model Architectures and Trends}{5}{subsection.1.3.1}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2}Datasets for Fine-Tuning and Benchmarking}{5}{subsection.1.3.2}\protected@file@percent }
\citation{russell2018automated}
\citation{NIST_SARD}
\citation{li2022sevc}
\citation{chen2023diversevul}
\citation{tihanyi_how_2024}
\citation{fan2020bigvul}
\citation{ding_vulnerability_2024}
\citation{li2022_vuldeelocator}
\citation{2024nistjulietc}
\citation{li2018vuldeepecker}
\citation{2024nistjulietjava}
\citation{luo2024fellmvp}
\citation{guru2021cvefixes}
\citation{10.1007/978-3-031-68738-9_34}
\citation{wang2022_vcmatch}
\citation{he2023_large}
\citation{ponta2019_manually}
\citation{gao_how_2023}
\citation{ullah_llms_2024}
\citation{ferreira2024-smartbugs}
\citation{ahmad2024_magma}
\citation{kouliaridis_assessing_2024}
\citation{wei2022chain}
\citation{sheng2025large}
\citation{tihanyi_how_2024}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces Datasets for Benchmarking and Fine-Tuning in Vulnerability detection}}{6}{table.caption.4}\protected@file@percent }
\newlabel{tab:datasets}{{1}{6}{Datasets for Benchmarking and Fine-Tuning in Vulnerability detection}{table.caption.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3}Prompt-Based Approaches}{6}{subsection.1.3.3}\protected@file@percent }
\citation{steenhoek2024err,299557}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.4}Emerging Trends and Ongoing Challenges}{7}{subsection.1.3.4}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {4}Formal Verification}{7}{section.1.4}\protected@file@percent }
\citation{MC1}
\citation{MC2}
\citation{Clarke2012}
\citation{BMCfirst}
\citation{ARM}
\citation{sousa2023lsverifier}
\citation{10458667}
\citation{pmlr-v202-pei23a}
\@writefile{toc}{\contentsline {section}{\numberline {5}Hybrid Approaches}{8}{section.1.5}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {5.1}LLM-Assisted Formal Verification}{8}{subsection.1.5.1}\protected@file@percent }
\citation{liu2024propertygpt}
\citation{lin2025fvel}
\citation{liu2024propertygpt}
\citation{curaba2024cryptoformaleval}
\citation{wu2023lemur}
\citation{tihanyi2023new}
\citation{liu2024propertygpt}
\citation{curaba2024cryptoformaleval}
\citation{tihanyi2023new}
\bibstyle{plain}
\bibdata{reference}
\bibcite{guru2021cvefixes}{1}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2}End-to-End Hybrid Pipelines}{10}{subsection.1.5.2}\protected@file@percent }
\bibcite{BMCfirst}{2}
\bibcite{chen2023diversevul}{3}
\bibcite{MC1}{4}
\bibcite{Clarke2012}{5}
\bibcite{curaba2024cryptoformaleval}{6}
\bibcite{sousa2023lsverifier}{7}
\bibcite{ding_vulnerability_2024}{8}
\bibcite{Formalverification}{9}
\bibcite{du2024generalization}{10}
\bibcite{fan2020bigvul}{11}
\bibcite{10.1145/3650212.3685304}{12}
\bibcite{ferrag2023securefalcon}{13}
\bibcite{ferreira2024-smartbugs}{14}
\bibcite{2024nistjulietc}{15}
\bibcite{2024nistjulietjava}{16}
\bibcite{gao_how_2023}{17}
\bibcite{hanif2022vulberta}{18}
\bibcite{ahmad2024_magma}{19}
\bibcite{he2023_large}{20}
\bibcite{jiang2024investigating}{21}
\bibcite{LLMfuzz}{22}
\bibcite{10458667}{23}
\bibcite{kouliaridis_assessing_2024}{24}
\bibcite{li2022_vuldeelocator}{25}
\bibcite{li2022sevc}{26}
\bibcite{li2018vuldeepecker}{27}
\bibcite{lin2025fvel}{28}
\bibcite{staticanalysis2022}{29}
\bibcite{liu2024propertygpt}{30}
\bibcite{luo2024fellmvp}{31}
\bibcite{lyu2024automatic}{32}
\bibcite{fuzzing}{33}
\bibcite{MECHRI2025104151}{34}
\bibcite{ESBMC}{35}
\bibcite{NIST_SARD}{36}
\bibcite{IAST}{37}
\bibcite{pmlr-v202-pei23a}{38}
\bibcite{invariants}{39}
\bibcite{ponta2019_manually}{40}
\bibcite{MC2}{41}
\bibcite{299557}{42}
\bibcite{roychoudhury2025ai}{43}
\bibcite{russell2018automated}{44}
\bibcite{sheng2025large}{45}
\bibcite{steenhoek2024err}{46}
\bibcite{10825051}{47}
\bibcite{tihanyi_how_2024}{48}
\bibcite{tihanyi2023new}{49}
\bibcite{10.1007/978-3-031-68738-9_34}{50}
\bibcite{ullah_llms_2024}{51}
\bibcite{pentest}{52}
\bibcite{wang2024your}{53}
\bibcite{wang2022_vcmatch}{54}
\bibcite{wei2022chain}{55}
\bibcite{wu2023lemur}{56}
\bibcite{ARM}{57}
\bibcite{zhou2024large}{58}
\bibcite{RASP}{59}
\gdef\minted@oldcachelist{,
  default.pygstyle,
  listing1.pygtex,
  listing2.pygtex}
\gdef \@abspage@last{15}

